Multi-Task Reinforcement Learning for Quadrotors

Reinforcement learning (RL) has shown great effectiveness in quadrotor control, enabling specialized policies to develop even human-champion-level performance in single-task scenarios. However, these specialized policies often struggle with novel tasks, requiring a complete retraining of the policy from scratch. To address this limitation, this paper presents a novel multi-task reinforcement learning (MTRL) framework tailored for quadrotor control, leveraging the shared physical dynamics of the platform to enhance sample efficiency and task performance. By employing a multi-critic architecture and shared task encoders, our framework facilitates knowledge transfer across tasks, enabling a single policy to execute diverse maneuvers, including high-speed stabilization, velocity tracking, and autonomous racing. Our experimental results, validated both in simulation and real-world scenarios, demonstrate that our framework outperforms baseline approaches in terms of sample efficiency and overall task performance.

==> equations/torques.tex <==
\begin{equation}
	\bm{\tau}_B = \begin{bmatrix}
		-d_{x_0}&-d_{x_1}&d_{x_2}&d_{x_3}\\
		d_{y_0}&-d_{y_1}&-d_{y_2}&d_{y_3}\\
		-c_{\tau}&c_{\tau}&-c_{\tau}&c_{\tau}
	\end{bmatrix}\begin{bmatrix}
		c_1\\c_2\\c_3\\c_4
	\end{bmatrix},
\end{equation}

==> figures/eyecatcher.tex <==
\makeatletter
\g@addto@macro\@maketitle{
  \captionsetup{type=figure}\setcounter{figure}{0}
  \def\mycolspace{1.2mm}
  \centering
  \vspace{5mm}
  \tikzset{font=\small}
  \begin{tikzpicture}    
    \node [inner sep=0pt, outer sep=0pt] (img1) at (0.3,0) 
    {\includegraphics[width=0.33\linewidth]{figures/jpg/hover.jpg}};
    \node [inner sep=0pt, outer sep=0pt, right=1mm of img1] (img2)
    {\includegraphics[width=0.33\linewidth]{figures/jpg/fig8.jpg}};
    \node [inner sep=0pt, outer sep=0pt, right=1mm of img2] (img3)
    {\includegraphics[width=0.33\linewidth]{figures/jpg/random_tracking.jpg}};
    % \node [inner sep=0pt, outer sep=0pt, below=2mm of img3] (text) {\text{(c) Velocity tracking}};
    % \node [inner sep=0pt, outer sep=0pt, below=2mm of img2] (text1) {\text{(b) Autonomous racing }};
    % \node [inner sep=0pt, outer sep=0pt, below=2mm of img1] (text2) {\text{(a)  Stabilizing from high speed}};

\end{tikzpicture}
    \vspace{0.5ex}
	\captionof{figure}{Control of a high-performance quadrotor through multi-task reinforcement learning. (Left): Stabilization from high speed; (Middle): Racing; (Right) Velocity tracking. The quadrotor is controlled using one neural network control policy. }
\vspace{-2pt}
\label{fig:catcheye}
}
\makeatother

==> figures/eyecatcher_second.tex <==
\begin{figure*}[t!]
  \begin{tikzpicture}    
    \node [inner sep=0pt, outer sep=0pt] (img1) at (0.3,0) 
    {\includegraphics[width=0.33\linewidth]{figures/jpg/hover.jpg}};
    \node [inner sep=0pt, outer sep=0pt, right=1mm of img1] (img2)
    {\includegraphics[width=0.33\linewidth]{figures/jpg/fig8.jpg}};
    \node [inner sep=0pt, outer sep=0pt, right=1mm of img2] (img3)
    {\includegraphics[width=0.33\linewidth]{figures/jpg/random_tracking.jpg}};
    \node [inner sep=0pt, outer sep=0pt, below=2mm of img3] (text) {\text{(c) Velocity tracking}};
    \node [inner sep=0pt, outer sep=0pt, below=2mm of img2] (text1) {\text{(b) Autonomous racing }};
    \node [inner sep=0pt, outer sep=0pt, below=2mm of img1] (text2) {\text{(a)  Stabilizing from high speed}};

\end{tikzpicture}
    \vspace{1.0ex}
	\captionof{figure}{The proposed approach performs three distinct tasks for quadrotor control in the real world. The resulting single MTRL policy can (a) track randomly generated velocities, (b) autonomously race through a fixed track, and (c) stabilize the platform after high-speed maneuvers.}
\label{fig:catcheye}
\end{figure*}

==> sections/white_paper.tex <==
\section{White Paper}
\begin{itemize}
    \item What is the problem?
    \item Why is it important?
    \item Why is the problem hard? What makes it challenging?
    \item How far has existing work come? What is the next frontier?
    \item Why hasn’t the problem been solved? What is the stumbling block?
    \item What does our paper contribute?
    \item What is the key idea? What is the magic trick? What is the new insight or technique that enables us to advance the frontier?
    \item What do the experiments say?
\end{itemize}

\subsection{What is the Problem?}
In this work, we introduce a multi-task reinforcement learning (MTRL) framework designed to enable a quadrotor to perform various agile and challenging tasks efficiently.

\subsection{Why is it important?}
Agile quadrotors are required to handle diverse missions ranging from search and rescue to infrastructure inspection.
%
These operations often involve a variety of specific tasks, such as tracking moving objects, maintaining stable hover positions, and following designated paths or objects.
%
Training a generalist policy to master these varied tasks can significantly enhance the versatility and adaptability of quadrotors, making them more effective for real-world applications.
%
In this work, we address the problem using deep reinforcement learning (RL), which offers the advantage of automatically optimizing parametric controllers through trial and error. 
%
RL effectively handles highly non-linear dynamical systems and non-convex objectives, which are typically challenging for conventional robotics methods. 
%
It has demonstrated significant success in agile quadrotor control.

\subsection{Why is the problem hard? What makes it challenging?}
%
State-of-the-art robot learning algorithms have demonstrated specialization with great performance, even outperforming humans in single-task scenarios~\cite{kaufmann2020deep}.
%
However, these specialist policies frequently struggle to generalize to novel, out-of-distribution tasks and always require training from scratch when faced with even minor changes in task configuration.
%
Hence, the commonly used task-specific training approach is unsuitable for multi-task scenarios. Developing a multi-task RL policy for quadrotors remains to be a significant challenge.
%

\subsection{How far has existing work come? What is the next frontier?}
%
Multi-task reinforcement learning has primarily been implemented in simulation environments, particularly in tasks like manipulation on the Meta-World benchmark~\cite{yu2020meta}.
%
In~\cite{kalashnikov2022scaling}, a large-scale collective robotic learning system, can rapidly acquire diverse skills by sharing exploration, experience, and representations across tasks, improving overall performance and capabilities.
%
~\cite{gupta2021reset} demonstrates using MT-RL to perform complex robotic skills like in-hand manipulation autonomously, significantly reducing the need for human resets during training sessions.
%
~\cite{yang2020multi} explores modularization in network design to facilitate MT-RL, improving both sample efficiency and the performance of robotic tasks by dynamically configuring network modules according to the task requirements.
%
~\cite{xie2022lifelong} explores a sequential multi-task learning scenario where a robot incrementally learns various tasks, using experiences from previous tasks to reduce the need for relearning and improve efficiency. 
%
~\cite{d2020sharing}  develops a general representation of features common across these tasks. This shared representation not only streamlines the learning process but also enhances the learning performance of individual tasks.
%

\subsection{Why hasn’t the problem been solved? What is the stumbling block?}
%
However, multi-task RL in the real world on quadrotors is largely unexplored.
%
One key factor distinguishing MTRL performance is the sharing of knowledge between different tasks to ensure information transfer across them. 
%
While the task-oriented objective remains consistent from one task to another, the underlying physical dynamics for the quadrotor platform, such as mass inertia and other physical properties, stay invariant throughout the learning process.
%
Hence, designing a functional MTRL framework and efficiently sharing information are the primary goals of this work.

\subsection{What does our paper contribute?}
In this paper, we propose the first multi-task reinforcement learning (MTRL) algorithm designed for quadrotor control. 

\subsection{What is the key idea? What is the magic trick? What is the new insight or technique that enables us to advance the frontier?}
The reinforcement learning framework employs a multi-critic setup, and we propose a shared task encoder for observations containing dynamical information while separating task-specific observations into a task-encoding network
%
By sharing common information and isolating task-specific data, we have developed a high-performance policy capable of executing maneuvers such as hovering, velocity tracking, and racing.

\subsection{What do the experiments say?}
%
In the experiments, we first detail our task design for the reinforcement learning training. 
%
Then, we introduce our MTRL setup, which includes efficient knowledge sharing through a novel dynamic encoding. 
%
Validated in simulation, our approach demonstrated higher sample efficiency compared to other baseline approaches. 
%
Finally, we validate our approach in the real world, showcasing its performance.

